Finite-Sample Symmetric Mean Estimation with Fisher Information Rate

The mean of an unknown variance-$\sigma^2$ distribution $f$ can be estimated from $n$ samples with variance $\frac{\sigma^2}{n}$ and nearly corresponding subgaussian rate. When $f$ is known up to translation, this can be improved asymptotically to $\frac{1}{n\mathcal I}$, where $\mathcal I$ is the Fisher information of the distribution. Such an improvement is not possible for general unknown $f$, but [Stone, 1975] showed that this asymptotic convergence $\textit{is}$ possible if $f$ is $\textit{symmetric}$ about its mean. Stone's bound is asymptotic, however: the $n$ required for convergence depends in an unspecified way on the distribution $f$ and failure probability $\delta$. In this paper we give finite-sample guarantees for symmetric mean estimation in terms of Fisher information. For every $f, n, \delta$ with $n > \log \frac{1}{\delta}$, we get convergence close to a subgaussian with variance $\frac{1}{n \mathcal I_r}$, where $\mathcal I_r$ is the $r$-$\textit{smoothed}$ Fisher information with smoothing radius $r$ that decays polynomially in $n$. Such a bound essentially matches the finite-sample guarantees in the known-$f$ setting.

==> estimation_using_lee_valiant.tex <==

\subsection{Local Estimation}
First, we introduce the estimator from \cite{lee_valiant_estimator} that we will make use of in our local estimation algorithm.
\begin{theorem}[From \cite{lee_valiant_estimator}]
\label{thm:lee_valiant_estimator}
There exists an estimator that, given $\delta > 0$ and samples $X_1 , \dots, X_n$ where each $X_i$ has mean $\mu$ and variance $\sigma^2$, produces an estimate $\hat \mu$ of $\mu$, such that with probability $1 - \delta$,
\[
    |\hat \mu - \mu|\le \sigma \cdot \left(1 + O\left(\sqrt{\frac{\log \frac{1}{\delta}}{n}}\right) + O\left(\frac{\log\log\frac{1}{\delta}}{\log\frac{1}{\delta}}\right)\right) \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}
\]
%aHere, the $o(1)$ term tends to $0$ as long as $\left(\frac{\log \frac{1}{\delta}}{n}, \delta \right) \to 0$.
\end{theorem}
\begin{algorithm}[H]\caption{Local Estimation}
\label{alg:local_estimation}
\vspace*{3mm}
\paragraph{Input Parameters:}
\begin{itemize}
\item Failure probability $\delta$, Samples $x_1, \dots, x_n \sim f^*$, the symmetrized and clipped KDE score function $\wh s_r^\sym$, symmetrization point $\mu_1$
\end{itemize}
\begin{enumerate}
\item For each sample $x_i$, compute a perturbed sample $x'_i = x_i + \mathcal N(0,r^2)$ where all the Gaussian noise are drawn independently across all the samples.
\item Use the estimator from Theorem~\ref{thm:lee_valiant_estimator} to compute an estimate $\hat \eps$ of $\E_{x \sim f_r}\left[\wh s^\sym_r(x)/\I_r \right]$ from samples $\wh s_r^\sym(x_i')/\I_r$ for all $i$, with input failure probability $\delta$.
\item
Return $\hat \mu = \mu_1 - \hat \eps$.
\end{enumerate}
\end{algorithm}
\begin{assumption}
\label{assumption:local_estimation}
Let $f_r$ be the $r$-smoothed version of distribution $f^*$ in Algorithm~\ref{alg:local_estimation}, with Fisher information $\I_r$. For parameter $\gamma$, $\wh s_r^\sym$ satisfies that for symmetrization point $\mu_1 = \mu + \eps$,
\begin{align*}
    \left|\E_{x \sim f_r}\left[\wh s_r^\sym(x) \right]  - \eps \I_r\right| \lesssim \frac{\eps \I_r}{\sqrt{\gamma}} \quad \text{and} \quad \left|\E_{x \sim f_r}\left[\wh s_r^\sym(x)^2 \right] - \I_r \right| \lesssim \frac{\I_r}{\sqrt{\gamma}}
\end{align*}
\end{assumption}
\begin{theorem}[Local Estimation]
\label{thm:local_estimation}
    In Algorithm~\ref{alg:local_estimation}, let $f_r$ be the $r$-smoothed version of $f^*$, with score function $s_r$ and Fisher information $\I_r$. Suppose for parameter $\gamma$, and $\wh s^\sym, \mu_1$, Assumption~\ref{assumption:local_estimation} is satisfied. Then, with probability $1 - \delta$, the output $\hat \mu$ of Algorithm~\ref{alg:local_estimation} satisfies
   \[
   \left| \hat \mu - \mu \right| \le \left(1 + o(1)+ O\left(\frac{1}{\sqrt{\gamma}} \right)\right) \sqrt{\frac{2 \log \frac{1}{\delta}}{n \I_r}} + O\left(\frac{\eps}{\sqrt{\gamma}}\right)
   \]
   where the $o(1)$ tends to $0$ as $\left(\frac{\log \frac{1}{\delta}}{n}, \delta \right) \to 0$.
\end{theorem}
\begin{proof}
    First, by Theorem~\ref{thm:lee_valiant_estimator}, the estimate $\hat \eps$ satisfies that with probability $1-\delta$,
    \begin{align*}
        \left|\hat \eps -\frac{1}{\I_r} \E_{x \sim f_r}\left[ \wh s_r^\sym(x)\right] \right| \le \frac{1}{\I_r}\sqrt{\E_{x\sim f_r}\left[\wh s_r^\sym(x)^2 \right]}\cdot (1+o(1)) \cdot \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}
    \end{align*}
    where the $o(1)$ tends to $0$ as $\left(\frac{\log \frac{1}{\delta}}{n}, \delta \right) \to 0$. Then, by Assumption~\ref{assumption:local_estimation}, this implies that with probability $1 - \delta$,
    \begin{align*}
        \left| \hat \eps - \eps\right| \le (1 + o(1)) \sqrt{\frac{2 \log \frac{1}{\delta}}{n \I_r}\left(1 + O\left(\frac{1}{\sqrt{\gamma}} \right)\right)} + O\left(\frac{\eps}{\sqrt{\gamma}}\right)
    \end{align*}
    So, since $\mu_1 = \mu + \eps$ and $\hat \mu = \mu + \hat \eps$, we have the claim.
\end{proof}

\subsection{Global Estimation}
\begin{algorithm}[H]\caption{Global Estimation}
    \label{alg:global_estimation} 
    \paragraph{Input parameters:}
    \begin{itemize}
        \item Failure probability $\delta$, Samples $x_1, \dots, x_n \sim f^*$, smoothing parameter $r$, approximation parameter $\xi > 0$.
    \end{itemize}
    \begin{enumerate}
        \item First, use the first $n/\xi$ samples to compute an initial estimate $\mu_1$ of the mean $\mu$ by using the estimator in Theorem~\ref{thm:lee_valiant_estimator} with failure probability $\delta/\xi$.
        \item Use the next $n/\xi$ samples to compute the symmeterized, clipped KDE score $\wh s_r^\sym$ (as defined in \eqref{eq:symmetrized_kde_def}, symmetrized around the initial estimate $\mu_1$.
        \item Run Algorithm~\ref{alg:local_estimation} using the remaining $n - \frac{2n}{\xi}$ samples, and failure probability $\delta(1 - 2/\xi)$, and return the final estimate $\hat \mu$.
    \end{enumerate}
\end{algorithm}

\begin{corollary}
  Let $\eps = C(\frac{\log \frac{1}{\delta}}{n})^{0.01}$ for a sufficiently large constant $C$.  Let $f^*$ be an arbitrary symmetric distribution with variance $\sigma^2$ and mean $\mu$.  For $r \geq \eps \sigma$, we have
  \[
  \abs{\wh{\mu} - \mu} \leq (1 + \eps) \sqrt{\frac{2 \log \frac{2}{\delta}}{n \I_r}}
  \]
  with probability $1-\delta$.
\end{corollary}

\begin{theorem}
  Let $\eps = C(\frac{\log \frac{1}{\delta}}{n})^{0.01}$ for a sufficiently large constant $C$.  Define $w_t$ to be the width between the $t$th and $(1-t)$th quantile.  For $r := \eps w_{\eps^{10}}$, Algorithm XXX achieves:
  \[
  \abs{\wh{\mu} - \mu} \leq (1 + \eps) \sqrt{\frac{2 \log \frac{2}{\delta}}{n \I_r}}
  \]
  with probability $1-\delta$.
  
  (For $t = $, Algorithm XXX estimates $w_{2t}$, getting something between $w_t$ and $w_{3t}$, and uses that for its $r$.)
\end{theorem}

\begin{theorem}[Global Estimation]
Let $f^*$ be an arbitrary distribution, and let $f_r$ be the $r$-smoothed version of $f^*$, with score function $s_r$ and Fisher information $\I_r$.
Let $C < \xi < \left(\frac{n}{\log\frac{1}{\delta}} \right)^{1/4}$ for large enough constant $C > 3$ be a parameter, and suppose $\left(\sqrt{\xi} \frac{n}{\log \frac{1}{\delta}}\right)^{1/4 + \alpha} \le \gamma \le \left(\frac{n}{\xi\log \frac{1}{\delta}} \right)^{2/5 - \alpha}$ for some small enough constant $\alpha >0$. For any $r \le \sigma$ and $\frac{n}{\log \frac{1}{\delta}} \ge \xi \left(\frac{\gamma^{5/12} \sigma }{r} \right)^{6+\alpha}$, with probability $1 - \delta$, Algorithm~\ref{alg:global_estimation} outputs an estimate $\hat \mu$ with
\[
|\hat \mu - \mu| \le (1 + o(1)) \sqrt{\frac{2\log \frac{1}{\delta}}{n \I_r}}
\]
where the $o(1)$ term goes to $0$ as $\left( \frac{\log \frac{1}{\delta}}{n}, \delta, \frac{1}{\gamma}, \frac{1}{\xi} \right) \to 0$.
\end{theorem}

\begin{proof}
    Let $\eps = \mu_1 - \mu$. First, note that by Theorem~\ref{thm:lee_valiant_estimator}, $\eps$ satisfies that with probability $1 - \delta/\xi$,
    \begin{align*}
        |\eps| &\le \sigma \cdot (1 + o(1)) \cdot \sqrt{\frac{2 \xi \log \frac{\xi}{\delta}}{n}}\\
        &\le \sigma \cdot (1 + o(1)) \cdot \xi^{1/2 + \alpha} \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}
    \end{align*}
    We condition on Step $1$ succeeding so that the above holds. To obtain bounds on the expectation and variance of $\wh s^\sym$, we will now check that the following conditions required to invoke Corollary~\ref{cor:sym_kde_variance} and Lemma~\ref{lem:sym_kde_mean} hold:
    \begin{itemize}
        \item $|\eps| \le r/60$
        \item $|\eps| \le r^2 \sqrt{\frac{\I_r}{\gamma}}$
    \end{itemize}
    Note that $\frac{\log \frac{1}{\delta}}{n} \le 1$ and $\gamma \ge 1$. Note also that $\xi > \left(\frac{n}{\log \frac{1}{\delta}} \right)^{1/4} \ge \gamma$. So, by our setting of $n$, 
    \[
        r \ge \sigma \gamma^{5/12} \xi^{1/6} \left(\frac{ \log \frac{1}{\delta}}{n}\right)^{1/6} \gg \sigma\cdot (1 + o(1)) \cdot \xi^{1/2 + \alpha} \sqrt{\frac{2 \log \frac{1}{\delta}}{n}} \ge |\eps|
    \]
    so that $|\eps| \le r/60$.
    Similarly
    \begin{align*}
        r^2 \sqrt{\frac{\I_r}{\gamma}} &\ge \sigma^2 \gamma^{5/6} \xi^{1/3} \left(\frac{\log \frac{1}{\delta}}{n} \right)^{1/3} \sqrt{\frac{\I_r}{\gamma}}\\
        &\ge \frac{\sigma^2\gamma^{5/6} \xi^{1/3}}{\sqrt{\sigma^2 + r^2}} \left(\frac{\log \frac{1}{\delta}}{n} \right)^{1/3} \quad \text{since $\I_r \ge \frac{1}{\sigma^2 + r^2}$}\\
        &\ge \frac{\sigma}{2} \gamma^{5/6} \xi^{1/3} \left(\frac{\log \frac{1}{\delta}}{n} \right)^{1/3} \quad \text{since $r \le \sigma$}\\
        &\gg \sigma \cdot (1 + o(1)) \cdot \xi^{1/2 + \alpha} \sqrt{\frac{2 \log \frac{1}{\delta}}{n}} \quad \text{since $\frac{\log \frac{1}{\delta}}{n} \le 1$, and $\xi \ge \gamma \ge 1$}\\
        &\ge |\eps|
    \end{align*}
    Also, our choice of $n$ implies that
    \begin{align*}
        \frac{n}{\xi} \ge \left(\frac{\gamma^{5/12} \sigma}{r} \right)^{6 + \alpha/2} \log \frac{\xi}{\delta}
    \end{align*}
    So, we can invoke Corollary~\ref{cor:sym_kde_variance} and Lemma~\ref{lem:sym_kde_mean} to obtain the following bounds on the mean and second moment of $\wh s^{\sym}$ in Step 2, which hold with probability $1 - \frac{\delta}{\xi}$.
    \begin{align*}
        \left|\E_{x \sim f_r}\left[\wh s_r^\sym(x) \right] - \eps \I_r \right| \lesssim \frac{\eps \I_r}{\sqrt{\gamma}} \quad \text{and} \quad \left|\E_{x \sim f_r}\left[\wh s_r^\sym(x)^2 \right] - \I_r \right|\lesssim \frac{\I_r}{\sqrt{\gamma}}
    \end{align*}
    Conditioned on the above event, Assumption~\ref{assumption:local_estimation} is satisfied, so that for $n' = n\left(1 - \frac{2}{\xi} \right)$ and $\delta' = \delta\left(1 - \frac{2}{\xi} \right)$, by Theorem~\ref{thm:local_estimation}, our final estimate $\hat \mu$ satisfies that with probability $1 - \delta' = 1-\delta\left(1 - \frac{2}{\xi} \right)$,
    \begin{align*}
        |\hat \mu - \mu| &\le \left(1 + o(1) + O\left(\frac{1}{\sqrt{\gamma}} \right) \right) \sqrt{\frac{2 \log \frac{1}{\delta'}}{n' \I_r}} + O\left(\frac{\eps}{\sqrt{\gamma}} \right)\\
        &=\left(1 + o(1) + O\left(\frac{1}{\sqrt{\gamma}} \right) \right) \sqrt{\frac{2 \log \frac{1}{\delta}}{n \I_r}} + O\left(\frac{\eps}{\sqrt{\gamma}} \right)\\
    \end{align*}
    Finally, we bound $\frac{\eps}{\sqrt{\gamma}}$. We have,
    \begin{align*}
        \frac{\eps}{\sqrt{\gamma}} &\le \frac{\sigma}{\sqrt{\gamma}} \xi^{1/2 + \alpha} (1 + o(1))\sqrt{\frac{2\log\frac{1}{\delta}}{n}}\\
        &\le \frac{\sigma^2}{\sqrt{\gamma(\sigma^2 + r^2)}} \xi^{1/2 + \alpha} \cdot (1 + o(1)) \cdot \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}\\
        &\le \frac{\sigma^2 \sqrt{\I_r}}{\sqrt{\gamma}} \xi^{1/2 + \alpha} \cdot (1 + o(1)) \cdot \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}\\
        &\le \left(\sigma^2 \gamma^{5/6} \xi^{1/3} \left(\frac{\log \frac{1}{\delta}}{n} \right)^{1/3} \right) \frac{\sqrt{\I_r}\xi^{1/6 + \alpha}}{\gamma^{4/3}}\cdot (1+o(1))\cdot \left(\frac{2 \log \frac{1}{\delta}}{n} \right)^{1/6}\\
        &\le \frac{r^2 \sqrt{\I_r}\xi^{1/6 + \alpha}}{\gamma^{4/3}} \cdot (1 + o(1)) \cdot \left(\frac{2 \log \frac{1}{\delta}}{n} \right)^{1/6} \quad \text{by setting of $n$}\\
        &\le \frac{\xi^{1/6 + \alpha}}{\sqrt{\I_r} \gamma^{4/3}} \cdot (1 + o(1)) \cdot \left(\frac{2 \log \frac{1}{\delta}}{n} \right)^{1/6} \quad \text{since $\I_r \le \frac{1}{r^2}$}\\
        &\ll \sqrt{\frac{2 \log \frac{1}{\delta}}{n \I_r}} \quad \text{since $\gamma \ge \left(\sqrt{\xi} \frac{n}{\log \frac{1}{\delta}} \right)^{1/4 + \alpha}$}
        %&\le \frac{1}{\sqrt{\I_r} \gamma} \quad \text{since $\I_r \le \frac{1}{r^2}$}\\
    \end{align*}
    So we have shown that 
    \[
        |\hat \mu - \mu| \le (1 + o(1)) \sqrt{\frac{2 \log \frac{1}{\delta}}{n \I_r}}
    \]
    Thus, by a union bound, with probability $1 - \delta$ in total, the claim follows.
\end{proof}


==> k_power_old_stuff.tex <==
\subsection{Analyzing the Gaussian}

\textbf{Idea:} Instead of using Chebyshev, use $k$ moment inequality.
With probability at most $\frac{k^{k/2}}{t^k}$, $X \ge t \sigma$. So, we can bound the atypical region contribution by 
$\frac{k^{k/2}}{rt^k } \log N$
We need this to be smaller than $k^{k/2} \I^{k/2}$. So, we can set $t$ to be larger than $\frac{\log N}{\sqrt{\I} r} > \frac{\log^{1/k} n}{\sqrt{\I} r^{1/k}}$. Then, everything else just works out.




\subsection{Mixture of two Gaussians for KDE}

Mixture of two standard Gaussians distance $d$ from mean each.

\subsection{Width $z_r$ region with probability $1 - 1/t^2$}
Let $z_r$ be the width of some region $S$ with probability at least $1 - 1/t^2$ for $t = \left( \frac{\log N}{\sqrt{\I} r}\right)^{\frac{k}{2} (1 + \gamma)}$ for constant $\gamma > 0$. We will show a result in terms of this width.

\begin{lemma}[Atypical Region]
$$\E_{x \sim f}[(u(x) - \Tilde u(x))^k \1_{x \not \in S}] \ll \I^{k/2}$$
\end{lemma}

\begin{proof}
By definition of $S$, $$\Pr_{x \sim f}[x \not\in S] \le \frac{1}{t^2}$$
Since by definition of $\Tilde u$ in \eqref{eq:clipped_kde_def}, $|\Tilde u| \le \frac{1}{r} \log N$, we have
$$\E_{x \sim f}[|\Tilde u(x)|^k \1_{x \not\in S}]\lesssim \frac{1}{t^2 r^k} \log^k N$$

Since $t = \left( \frac{\log N}{\sqrt{\I} r}\right)^{\frac{k}{2} (1 + \gamma)}$, we have
$$\E_{x \sim f}[|\Tilde u(x)|^k \1_{x \not\in S}] \lesssim \frac{(\I^{k/2} r^k)^{1+\gamma}}{r^k (\log^k N)^{1+\gamma}} \log^k N \ll \I^{k/2}$$
Now, by Lemma~\ref{lem:set_k_power_bound}, we have
\end{proof}

\subsection{$k^{th}$ power scratch}
\begin{lemma}[$k$ power generic error estimate over large density region]
\label{lem:generic_error_estimate_large_density}
Let $N \gg \frac{\log \frac{1}{\delta} \log \frac{1}{\alpha r}}{\alpha r}$. Then, for the KDE $\wh u$ defined in \eqref{eq:kde_def}, with probability $1 - \delta$ over the samples $Y_1, \dots, Y_N \sim f^*$, we have that,
\begin{align*}
    \E_{x \sim f}[(\wh u(x) - u(x))^k \1_{|x - \mu| \le t \sigma \text{ and } f(x) \ge \alpha}] \lesssim \left(\frac{k\log \frac{\sqrt{\alpha N} t \sigma}{\sqrt{kr} \delta}}{\alpha N r^3}\right)^{k/2}
\end{align*}
%\begin{align*}

%    \E_{x \sim f}[(\wh u(x) - u(x))^2 1_{|x - \mu| \le t \sigma \text{ and } f(x) \ge \alpha}] \lesssim t \sigma \sqrt{\frac{\log \frac{1}{\delta}}{\alpha^3 r^9 N}}
%\end{align*}
\end{lemma}

\begin{proof}
For $i \in \left[0, \floor{\frac{2 t \sigma}{\eps}}\right]$, let $x_i'$ be the smallest $x$ such that $f(x) \ge \alpha$ in the region $\mu - t \sigma + i\eps $. Then, we have that $$\left\{x : |x - \mu| \le t \sigma \text{ and } f(x) \ge \alpha \right\} \subseteq\cup_{i=0}^{\floor{\frac{2 t \sigma}{\eps}} } [x_i'-\eps, x_i' + \eps]$$
   Now, $N \gg \frac{\log \frac{1}{\delta}}{\alpha r}$ and $\frac{\eps}{r} \sqrt{ \log \frac{1}{\alpha r}} = \sqrt{\frac{\log \frac{1}{\alpha r}}{r \alpha N}} \ll 1$. So, by the union bound, and Lemma \ref{lem:generic_error_estimate_within_bin}, we have that for all $x$ such that $|x - \mu| \le t \sigma$ and $f(x) \ge \alpha$,
   $$|\wh u(x) - u(x)| \lesssim \sqrt{\frac{\log \frac{t\sigma}{\eps \delta}}{\alpha N r^3}} + u(x) \sqrt{\frac{\log \frac{t \sigma}{\eps \delta}}{\alpha N r} } + \frac{\eps}{r^2}$$
   So, $$\E[(\wh u(x) - u(x))^k \1_{|x - \mu| \le t \sigma \text{ and } f(x) \ge \alpha}] \lesssim \left(\frac{\log \frac{t \sigma}{\eps \delta}}{\alpha N r^3}\right)^{k/2} + \E[u(x)^k \1_{|x - \mu| \le t\sigma \text{ and } f(x) \ge \alpha}] \left(\frac{\log \frac{t \sigma}{\eps \delta}}{\alpha N r}\right)^{k/2} + \frac{\eps^k}{r^{2k}}$$
   Using Lemma~\ref{lem:score-moments}, since $\I \le \frac{1}{r^2}$, we get
   $$\E[(\wh u(x) - u(x))^k \1_{|x - \mu| \le t \sigma \text{ and } f(x) \ge \alpha}] \lesssim \left(\frac{k\log \frac{t\sigma}{\eps \delta}}{\alpha N r^3} \right)^{k/2} + \frac{\eps^k}{r^{2k}}$$
   Plugging in $\eps = \sqrt{\frac{kr}{\alpha N}}$ gives the claim.
   %Choosing $\eps = r/\sqrt{N}$ gives the claim.
\end{proof}
\begin{lemma}[Error estimate over large density region (instantiated)]
\label{lem:k_power_error_estimate_large_density}
    Let $\gamma > 0$ be a small constant. Let $r \gg \frac{\sigma}{N^{1/(6 + \gamma)}} \log \frac{1}{I r^2} \log \frac{1}{\delta}$, $t = \left(\frac{\log \frac{1}{\I r^2}}{\sqrt{\I} r}\right)^{\frac{k}{2}(1 + \gamma)}$ and $\alpha = \frac{1}{t^2(t \sigma)}$. Then, for the KDE $\wh u$ defined in \eqref{eq:kde_def}, with probability $1 - \delta$ over the samples $Y_1, \dots, Y_N \sim f^*$, we have $$\E_{x \sim f}[(\wh u(x) - u(x))^2 1_{|x - \mu| \le t \sigma \text{ and } f(x) \ge \alpha}] \ll \I^{k/2}$$
\end{lemma}
\begin{proof}
    $\I \ge\frac{1}{\sigma^2}$. So, for our setting of $r, \alpha$ and $t$, $$N \gg \frac{\log \frac{1}{\delta} \log \frac{1}{\alpha r}}{\alpha r}$$
    So, the conditions of Lemma~\ref{lem:generic_error_estimate_large_density} are satisfied.
    So, the claim follows by plugging in $t, \alpha$ and $r$ into Lemma~\ref{lem:generic_error_estimate_large_density}.
\end{proof}
\begin{lemma}[$k$ power error estimate over small density regions within typical region]
XXX TODO: Are we losing something here?
\label{lem:error_estimate_small_density}
Let $\alpha = \frac{\I r^2}{t \sigma \log^2 \frac{1}{\I r^2}}$. Then, for the KDE $\wh u$ defined in \eqref{eq:kde_def}, we have
    \begin{align*}
        \E_{x \sim f}[(\wh u(x) - u(x))^2 1_{|x - \mu| \le t \sigma \text{ and } f(x) \ll \alpha}] \ll \I
    \end{align*}
\end{lemma}
\begin{proof}
    First, $$\Pr[|x - \mu| \le t \sigma \text{ and } f(x) \ll \alpha] \ll \alpha t \sigma$$
    $$\E[u(x)^2 1_{|x - \mu| \le t \sigma \text{ and } f(x) \ll \alpha}] \ll \frac{\alpha t \sigma}{r^2} \log^2 \frac{1}{\alpha t \sigma}$$
    XXX REST NOT CORRECT
    So, by Corollary~\ref{cor:score_error_bounded_in_small_set}, we have $$\E[(\wh u(x) - u(x))^2 1_{|x - \mu| \le t \sigma \text{ and } f(x) \ll \alpha}] \ll \frac{\alpha t \sigma}{r^2} \log^2 \frac{1}{\alpha t \sigma}$$
    So, for our choice of $\alpha$, the right hand side is
    $$\frac{\I}{\log^2 \frac{1}{\I r^2}} \log^2\frac{\log ^2 \frac{1}{\I r^2}}{\I r^2} \lesssim \I$$
    The claim follows.
\end{proof}

%The below bound for a Gaussian:


\begin{lemma}[set $kth$ power bound]
\label{lem:set_k_power_bound}
For set $S$ with $\Pr[S] \le \beta$, and any $r$-smoothed distribution with score function $u$, for $r \le 1$, we have
$$\E_{x \sim f}[|u(x)|^k 1_{x \in S}] \lesssim \frac{(2e)^k\beta}{r^k}\left(k^{k/2} + \log^{k/2} \frac{1}{\beta}\right)$$
\end{lemma}
\begin{proof}
\begin{align*}
\E[|u(x)|^k \1_{x \in S}] &= \int_{0}^\infty \Pr[|u(x)|^k 1_{x \in S} \ge t] dt\\
&\le \int_{0}^\infty \min(\Pr[x \in S], \Pr[|u(x)|^k \ge t]) dt\\
&\le \int_0^\infty \min(\beta, \Pr[|u(x)| \ge t^{1/k}])dt
\end{align*}
By Lemma~\ref{lem:score-moments}, since $\I \le \frac{1}{r^2}$, this is
\begin{align*}
    &\lesssim \int_0^\infty \min(\beta, e^{-t^{2/k} r^2} ) dt\\
    &\lesssim \frac{\beta}{r^k} \log^{k/2} \frac{1}{\beta} + \int_{\frac{1}{r^k} \log^{k/2} \frac{1}{\beta}}^\infty e^{-t^{2/k} r^2} dt\\
    &= \frac{\beta}{r^k} \log^{k/2} \frac{1}{\beta} + \frac{k}{2 r^k} \int_{\log\frac{1}{\beta}}^\infty e^{-u} u^{k/2 - 1} du\\
    %&\lesssim \beta \log \frac{1}{\beta} + \frac{k}{2r^k}\int_{\log \frac{1}{\beta}}^\infty e^{-u} u^{\frac{k}{2} - 1} du\\
    %&\lesssim \beta B + \int_B^\infty e^{-t^{2/k} r^2} dt\\
        %&\lesssim \beta B + \frac{1}{r^k} e^{-r^2 B^{2/k}} k^k \frac{1}{\frac{k - \frac{r^{2} B^{i/k}}{k}}
\end{align*}

 We have that for $k\ge 2$, $B \ge k$,
 \begin{align*}
     e^{-(B + 2)} (B + 2)^{k/2 - 1} &= B^{k/2 - 1} e^{-B} \left(e^{-2} \left(1 + \frac{2}{B}\right)^{k/2 - 1} \right)\\
     &\le B^{k/2 - 1} e^{-B} \left(e^{-2} e^{\frac{2}{B} (\frac{k}{2} - 1)} \right) \\
     &\le \frac{B^{k/2 - 1} e^{-B}}{e}
 \end{align*}
%\begin{align*}
%e^{-(B+x)} (B+x)^{\frac{k}{2} - 1} &= B^{k/2 - 1} e^{-B} \left(e^{-x} \left(1 + \frac{x}{B} \right)^{k/2 - 1}  \right)\\
%&\le B^{k/2 - 1} e^{-B} \left(e^{-x} e^{\frac{x}{B} (k/2 - 1)} \right)\\
%&\le \frac{B^{k/2 - 1} e^{-B}}{e}
%\end{align*}
%where the last line follows since $-x + \frac{x}{B} (k/2 - 1) \le -\frac{x}{2} = -1$

%Now, 
%\begin{align*}
%    \int_{k/2}^\infty e^{-u} u^{k/2 - 1} du &= \int_{k/2}^k e^{-u} u^{k/2 - 1} du + \int_k^\infty e^{-u} u^{k/2 - 1} du\\
%    &\le  e^{-k/2} \left(\frac{k}{2}\right)^{k/2} + \sum_{i=0}^\infty \int_{k + 2i}^{k+2(i+1)} e^{-u} u^{k/2 - 1} du\\
%\end{align*}
So, for $\beta \le e^{-k}$, we have
\begin{align*}
    \int_{\log\frac{1}{\beta}}^\infty e^{-u} u^{k/2 - 1} du &= \sum_{i=0}^\infty \int_{\log\frac{1}{\beta} + 2i}^{\log \frac{1}{\beta} + 2 (i+1)} e^{-u} u^{k/2 - 1} du\\
    &\le 2 \sum_{i=0}^\infty \frac{\beta \log^{k/2 - 1} \frac{1}{\beta}}{e^i} \\
    &\lesssim \beta \log^{k/2 - 1} \frac{1}{\beta}\\
\end{align*}
For $e^{-k} \le \beta \le e^{-k/2 +1}$,
\begin{align*}
    \int_{\log \frac{1}{\beta}}^\infty e^{-u} u^{k/2 - 1} du &= \int_{\log \frac{1}{\beta}}^k e^{-u} u^{k/2 - 1} du + \int_k^\infty e^{-u} u^{k/2 - 1} du\\
    &\lesssim \frac{k}{2} \beta \log^{k/2 - 1} \frac{1}{\beta} + e^{-k} k^{k/2 - 1}\\
    &\lesssim \frac{k}{2} \beta \left(\log^{k/2 - 1} \frac{1}{\beta} + k^{k/2 - 1} \right)
    %&\lesssim k^{k/2 - 1} \beta \log^{k/2 - 1} \frac{1}{\beta}
\end{align*}

For $\beta \ge e^{-(k/2 - 1)}$, we have
\begin{align*}
    \int_{\log \frac{1}{\beta}}^\infty e^{-u} u^{k/2 - 1} du &\le \int_0^\infty e^{-u} u^{k/2 - 1} du\\
    &= k^{k/2-1}\\
    &\le \beta \frac{k^{k/2 - 1}}{\beta}\\
    &\le \beta k^{k/2-1} e^{k/2 - 1}\\
\end{align*}

So, for $\beta \le e^{-k}$, and $\beta \ge e^{-k/2 + 1}$, the claim follows immediately. For $e^{-k} \le \beta \le e^{-k/2 + 1}$, using $k \le 2^k$ for all $k \ge 2$, the claim follows. 

%So integrate from 0 to infinity, get something like $k^{k/2}$.
%Issue is that this is not $\beta k^{k/2}$.
%So instead, we say that $k^{k/2} = \beta k^{k/2}/\beta \le \beta k^{k/2} e^{k/2-1}$.
%
%
%For $e^{-k/2 + 1} \le \beta \le e^{-k/4 + 1/2}$,
%\begin{align*}
%    \int_{\log \frac{1}{\beta}}^\infty e^{-u} u^{k/2 - 1} du &= \int_{\log \frac{1}{\beta}}^{k/2 - 1} e^{-u} u^{k/2 - 1} du + \int_{k/2 - 1}^\infty e^{-u} u^{k/2 - 1} du\\
%    &\lesssim \left(\frac{k}{4} + \frac{1}{2}\right) \beta \log^{k/2} \frac{1}{\beta} + e^{-k/2 + 1}k^{k/2} 
%\end{align*}
%XXX \textbf{second term above is a problem}
%
%Now, when $k \ge 3$, $B \le k/4 - 1/2$,
%\begin{align*}
%    e^{-(B - 2)} (B - 2)^{k/2 - 1} &\le B^{k/2 - 1} e^{-B} \left( e^{2} e^{-\frac{2}{B} (\frac{k}{2} - 1)}\right)\\
%    &\le \frac{B^{k/2 - 1} e^{-B}}{e^2}\\
%\end{align*}
%So, for $\beta \ge e^{-k/4 + 1/2}$
%
%\begin{align*}
%    \int_{\log \frac{1}{\beta}}^{k/4 - 1/2} e^{-u} u^{k/2 - 1} du &= \sum_{i=0}^\infty \int_{k/4 - 1/2 - 2i}^{k/4 - 1/2 - 2(i+1)} e^{-u} u^{k/2 - 1} du\\
%    &\le 2 e^{-k/4+1/2} (k/4 - 1/2)^{k/2 - 1} \sum_{i=0}^\infty e^{-2i}\\
%    &\lesssim e^{-k/4 + 1/2} (k/4 - 1/2)^{k/2 - 1}\\
%    &\lesssim \beta k^{k/2 - 1}\\
%\end{align*}
%
%So for $\beta \ge e^{-k/4 + 1/2}$,
%\begin{align*}
%    \int_{\log \frac{1}{\beta}}^{\infty} e^{-u} u^{k/2 - 1} du &= \int_{\log \frac{1}{\beta}}^{k/4 - 1/2} e^{-u} u^{k/2 - 1} du + \int_{k/4 - 1/2}^\infty e^{-u} u^{k/2 - 1} du\\
%    &\lesssim \beta k^{k/2 - 1} + e^{-k/2 + 1} k^{k/2 - 1}\\
%    &\lesssim \beta k^{k/2 - 1}\\
%\end{align*}
%
%XXX More Scratch:
%\textbf{Factor $k$ loss:} The above loses a factor of $k$, because the integral near $u = k/2 - 1$ is not approximated tightly enough. We want to approximate
%
%$$\int_{k/2 - 1}^k e^{-u} u^{k/2 - 1} du$$
%
%Above, we just approximated this naively by $\left(k/2 + 1 \right)e^{-k/2 + 1} \left(k/2 - 1 \right)^{k/2 - 1}$, but note that this incurs a factor $k$ loss. Trying the same half life idea here more carefully:
%
%\begin{align*}
%e^{-k/2 + 1 - c} \left(k/2 - 1 + c \right)^{k/2 - 1} &= e^{-k/2 + 1} \left(k/2 - 1 \right)^{k/2 - 1} e^{-c} \left(\frac{k/2 - 1 + c}{k/2 - 1} \right)^{k/2 - 1}\\
%\end{align*}
%
%Now, looking at the factor, and approximating up to the second order term gives
%\begin{align*}
%    e^{-c} \left(1 + \frac{c}{k/2 - 1} \right)^{k/2 - 1} \approx 1 - \frac{c^2}{k - 2}
%\end{align*}
%Setting this to a constant $< 1$ gives that $c \approx O(\sqrt{k})$. But this approximation still incurs a $\sqrt{k}$ loss.
%
%Calculation from above:
%\begin{align*}
%    e^{-c} \left(1 + \frac{c}{k/2 - 1} \right)^{k/2 - 1} &\le \left(1 - c + \frac{c^2}{2} \right) \left(1 + c + \binom{k/2 - 1}{2} \left(\frac{c}{k/2 - 1} \right)^2 \right)\\
%    &= 1 - \frac{c^2}{k- 2} + blah
%\end{align*}
%
%\textbf{Using this bound:} If we get $k^{k/2}$, this will give us 
%$$\E[(\Tilde u - u)^k] \ll \I^{k/2} k^{k/2}$$
%
\end{proof}
XXX Scratch
Now, we want a bound on $\E[|\Tilde u|^k]$ that matches Lemma~\ref{lem:score-moments}.

\begin{align*}
    \E[|\Tilde u|^k] &= \E[|\Tilde u - u + u|^k]\\
    &\le \sum_{i=0}^k \binom{k}{i} \E[|\Tilde u - u|^i |u|^{k-i}]\\
\end{align*}
By Holder's inequality, this is
\begin{align*}
    &\le \sum_{i=0}^k \binom{k}{i} \E[|\Tilde u - u|^k]^{i/k} \E[|u|^k]^{\frac{k-i}{k}}\\
 \end{align*}

Now, 
\begin{align*}
    \sum_{i=0}^{k-1} \binom{k}{i} \E[|\Tilde u - u|^k]^{i/k} \E[|u|^k]^{\frac{k-i}{k}} &\ll \sum_{i=0}^{k-1} \binom{k}{i} k^{i/2} \I^{i/2} \left((c/r)^{k-2} k^{k/2} \I \right)^{\frac{k-i}{k}}\\
    &\ll 2^k k^{k/2}\left(\frac{c}{r}\right)^{k-2} \I\\
\end{align*}



\subsection{k power}
\begin{lemma}[Atypical region]
\label{lem:k_power_atypical_region}
Let $N \gg \frac{\log \frac{1}{\delta} \log \frac{1}{\alpha r}}{\alpha r}$. For the clipped KDE $\Tilde u$ defined in \ref{eq:clipped_kde_def}, with probability $1 - \delta$ over the samples $Y_1, \dots, Y_n \sim f^*$, we have
$$\E_{x \sim f}[(u(x) - \Tilde u(x))^k \1_{|x - \mu| \ge t \sigma}] \ll \I^{k/2}$$
for $t = \left(\frac{\log n}{\sqrt{\I} r} \right)^{\frac{k}{2}(1+ \gamma)}$ for small constant $\gamma > 0$.
\end{lemma}

\begin{proof}
By Chebyshev's inequality,
$$\Pr[|x - \mu| \ge t \sigma] \le \frac{1}{t^2}$$
Since by the definition of $\Tilde u$ in \ref{eq:clipped_kde_def} $|\Tilde u|$ is clipped at $\frac{1}{r} \log n$, we have
$$\E_{x \sim f}[|\Tilde u(x)|^k \1_{|x - \mu| \ge t \sigma}] \lesssim \frac{1}{t^2 r^k} \log^k n = \frac{(\I^{k/2} r^k)^{1 + \gamma}}{r^k (\log^k n)^{1 + \gamma}} \log^k n \le \frac{\I^{k/2}}{\log^{k\gamma} n}}$$
where the last inequality follows from the fact that $\I \le \frac{1}{r^2}$.
Now, by Lemma~\ref{lem:set_k_power_bound}, we have
$$\E_{x \sim f}[|u(x)|^k \1_{|x - \mu| \ge t \sigma}] \lesssim \frac{2k^k}{t^2 r^k} \log^{k/2} t  \lesssim \frac{2 k^k (\I^{k/2} r^k)^{1+\gamma}}{(\log^{k(1+\gamma)} n) r^k} \log^{k/2}\left( \left(\frac{\log n}{\sqrt{\I} r} \right)^{\frac{k}{2}(1+\gamma)} \right)$$
XXX Complete proof (show relationship)
\end{proof}

\begin{lemma}[Typical small density region]
\label{lem:k_power_typical_small_density_region}
Let $N \gg \frac{\log \frac{1}{\delta} \log \frac{1}{\alpha r}}{\alpha r}$. For the clipped KDE $\Tilde u$ defined in \ref{eq:clipped_kde_def}, with probability $1 - \delta$ over the samples $Y_1, \dots, Y_n \sim f^*$, we have
$$\E_{x \sim f}[(u(x) - \Tilde u(x))^k \1_{|x - \mu| \le t \sigma \text{ and } f(x) \le \alpha}] \ll \I^{k/2}$$
for $t = \left(\frac{\log n}{\sqrt{\I} r} \right)^{\frac{k}{2}(1 + \gamma)}$ and $\alpha = \frac{1}{t^3 \sigma}$.
\end{lemma}

\begin{proof}
Since by definition of $\Tilde u$ in \ref{eq:clipped_kde_def}, $|\Tilde u|$ is clipped at $\frac{1}{r} \log n$, we have
$$\E_{x \sim f}[|\Tilde u(x)|^k \1_{|x - \mu| \ge t \sigma}] \lesssim \frac{\alpha t \sigma}{r^k} \log^k n = \frac{1}{t^2 r^k} \log^k n \ll \I^{k/2}$$
Now, by Lemma~\ref{lem:set_k_power_bound},
$$\E_{x \sim f}[|u(x)|^k \1_{|x - \mu| \le t \sigma \text{ and } f(x) \le \alpha}] \le \frac{\alpha t \sigma k^k}{r^k} \log^{k/2} \frac{1}{\alpha t \sigma} \le \frac{2 k^k}{r^k t^2} \log^{k/2} t \ll \I^{k/2}$$
The claim follows
\end{proof}

\begin{lemma}[Typical large density region]
\label{lem:k_power_typical_large_density_region}
Let $N \gg \frac{\log \frac{1}{\delta} \log \frac{1}{\alpha r}}{\alpha r}$. For the clipped KDE $\Tilde u$ defined in \ref{eq:clipped_kde_def}, with probability $1 - \delta$ over the samples $Y_1, \dots, Y_n \sim f^*$, we have
$$\E_{x \sim f}[(u(x) - \Tilde u(x))^k \1_{|x - \mu| \le t \sigma \text{ and } f(x) \ge \alpha}] \ll \I^{k/2}$$
\end{lemma}

\begin{proof}
First, by Lemma~\ref{lem:generic_density_large_score_small}, for $x$ such that $f(x) \ge \alpha$,
\begin{align*}
|u(x)| &\le \frac{1}{r} \sqrt{2 \log \frac{1}{\sqrt{2 \pi} r \alpha} } \le \frac{1}{r} \sqrt{2 \log\left(\frac{\sigma}{\sqrt{2 \pi}r} \left(\frac{\log n}{\sqrt{\I} r}\right)^{3+3\gamma} \right)}\\
&\le \frac{1}{r} \sqrt{2 \log \left(\log^{3 + 3\gamma} n \right) + 2 \log \frac{\sigma }{\sqrt{2 \pi} r (\sqrt{\I} r)^{3 + 3 \gamma}} }\\
\end{align*}
Now, since $\I \ge \frac{1}{\sigma^2}$, this gives
\begin{align*}
    |u(x)| \le \frac{1}{r} \sqrt{2 \log (\log^{3 + 3\gamma} n) + 2 \log \frac{\sigma^{4 + 3 \gamma}}{\sqrt{2 \pi} r^{4 + 3\gamma}} }
\end{align*}
Now, since $r \gg \sigma/\text{poly}(N)$, this gives finally that, when $f(x) \ge \alpha$,
$$|u(x)| \le \frac{1}{r} \log N$$

Then, since $|\Tilde u|$ is clipped at $\frac{1}{r} \log N$ as per definition \eqref{eq:clipped_kde_def}, by Lemma~\ref{lem:k_power_error_estimate_large_density}, we have the claim.

\end{proof}
\begin{theorem}[KDE score is close to true score ($k^{th}$ power)]
\label{thm:k_power_kde_score_close_to_true_score}
Let $\gamma > 0$ be a small constant. Let $r \gg \frac{\sigma\log \frac{1}{\delta}}{N^{1/(6 + \gamma)}} $. Then, for the clipped KDE $\Tilde u$ defined in \eqref{eq:clipped_kde_def}, with probability $1 - \delta$ over the samples $Y_1, \dots, Y_N \sim f^*$, we have
    $$\E_{x \sim f}[(\Tilde u(x) - u(x))^k] \ll \I^{k/2}$$
\end{theorem}

\begin{proof}
\begin{align*}
 \E[(\wh u(x) - u(x))^k] &= \E[(\wh u(x) - u(x))^k (1_{|x - \mu| \le t \sigma} + 1_{|x - \mu| > t\sigma})]\\
 &= \E[(\wh u(x) - u(x))^k (1_{|x - \mu| \le t \sigma \text{ and } f(x) \ge \alpha} + 1_{|x - \mu| \le t \sigma \text{ and } f(x) \ll \alpha})] \\
 &+ \E[(\wh u(x) - u(x))^k 1_{|x - \mu| > t \sigma}]
 \end{align*}
By Lemmas~\ref{lem:k_power_atypical_region},~\ref{lem:k_power_typical_small_density_region}, and \ref{lem:k_power_typical_large_density_region}, the claim follows.
\end{proof}


==> kde_two_sample_testing.tex <==

\section{Two-sample testing}
\paragraph{Problem Statement:} Given samples $x_1, \dots, x_n \sim f^*$ and $y_1, \dots, y_n \sim g^*$ where $g^*(x) = f^*(x - \beta)$ for all $x$, we want to test whether $\beta = 0$ or $|\beta| \ge \beta^*$.

\begin{algorithm}\caption{Biased estimator}
     \label{alg:testing_biased_estimator} 
    \paragraph{Input parameters:}
    \begin{itemize}
        \item Failure probability $\delta$, Samples $a_1, \dots, a_n$, clipped KDE score $\wh s_r^\clip$, approximation parameter $\xi$
    \end{itemize}
    \begin{enumerate}
        \item First, use the first $n/\xi$ samples to compute an initial estimate $\mu_1$ of the mean $\mu$ by using the Median-of-Means estimator in Lemma~\ref{lem:median_of_means} with failure probability $\delta/\xi$.
        \item Let the remaining $n(1 - 1/\xi)$ samples be $b_1, \dots, b_{n'}$. For each sample $b_i$, compute a perturbed sample $b_i' = b_i + \mathcal N(0, r^2)$, where all the Gaussian noise are drawn independently across all the samples.
        \item Compute $\wh \eps = \frac{1}{\I_r}$
        %\item Use the next $n/\xi$ samples to compute the symmeterized, clipped KDE score $\wh s_r^\sym$ (as defined in \eqref{eq:symmetrized_kde_def}), symmetrized around the initial estimate $\mu_1$.
        %\item Run Algorithm~\ref{alg:local_estimation_empirical_mean} using the remaining $n - \frac{2n}{\xi}$ samples, and failure probability $\delta(1 - 2/\xi)$, and return the final estimate $\hat \mu$.
    \end{enumerate}
\end{algorithm}

==> misc_rademacher_kde_notes.tex <==


\section{Rademacher Complexity}
For a function class $\mathcal F$, and $f(X_1), \dots, f(X_n)$ subgaussian with constant parameter for all $f \in \mathcal F$ we have that with probability $1 - e^{-\eps^2 n}$,
$$\sup_{f \in \mathcal F} |\sum_{i=1}^n \frac{1}{n} f(X_i) - \E[f(X)]| \le 2 \mathcal R_{\mathcal F} + \eps$$
where $$\mathcal R_{\mathcal F} = \E_{\sigma, X}\left[\sup_{f \in \mathcal F} \frac{1}{n} \sum_{i=1}^n \sigma_i f(X_i) \right]$$
is the Rademacher complexity of $\mathcal F$. Here $\sigma_i$ are sampled from $\{-1, +1\}$.

In our case, the function class $\mathcal F$ will be $s_r(x - \eps)$ for all $\eps \le \eps_\max$. (Here $x$ is $- \sqrt{\frac{\log \frac{1}{\delta}}{n} \I_r}$).
So, we have, with probability $1 - \delta$,
$$\sup_{\eps \le \eps_\max}|\sum_{i=1}^n \frac{1}{n} s_r(X_i - \eps) - \E[s_r(x - \eps)]| \le 2 \mathcal R_{\mathcal F} + \sqrt{\frac{\log \frac{1}{\delta}}{n} \I_r}$$

where $$\mathcal R_{\mathcal F} = \E_{\sigma, X} \left[\sup_{\eps \le \eps_\max} \frac{1}{n} \sum_{i=1}^n \sigma_i s_r(X_i - \eps) \right]$$
Suppose, to get a sense of things, that $s_r$ were really $\frac{1}{r^2}$-Lipschitz. Then,
$$|s_r(X_i - \eps) - s_r(X_i)| \le \frac{\eps}{r^2}$$
So, if we can show that for a fixed $X_i, \sigma_i$, that for \emph{every} $\eps$, we have
$$\sigma_i s_r(X_i) - \frac{\eps}{r^2} \le \sigma_i s_r(X_i - \eps) \le \sigma_i s_r(X_i) + \frac{\eps}{r^2}$$
then, we are ok. We know that when $\sigma_i = 1$, this is just true. When $\sigma_i = -1$, since $s_r(X_i - \eps) \le s_r(X_i) + \eps/r^2$, we have
$$\sigma_i s_r(X_i - \eps) \ge \sigma_i s_r(X_i) - \eps/r^2$$
Similarly, $$\sigma_i s_r(X_i - \eps) \le \sigma_i s_r(X_i) + \eps/r^2$$
So, the claim is true. 
\begin{align*}
    \mathcal R_{\mathcal F} \le \sqrt{\E_{\sigma, X} \left[\sup_{\eps \le \eps_\max} \left(\frac{1}{n} \sum \sigma_i s_r(X_i - \eps) \right)^2 \right]}
\end{align*}
By independence of $X_i, \sigma_i$, and since $\sigma_i \in \{-1, 1\}$, this is at most
\begin{align*}
&\frac{1}{n} \sqrt{\E_{X} \left[ \sup_{\eps \le \eps_\max}\sum_{i=1}^n s_r(X_i - \eps)^2  \right] }\\
&\le \frac{1}{n} \sqrt{\E_X\left[\sup_{\eps \le \eps_\max} \sum_{i=1}^n (s_r(X_i) + \frac{\eps}{r^2})^2 \right] }\\
&\lesssim \frac{1}{n} \sqrt{\E\left[\sum_{i=1}^n s_r(X_i)^2 \right] + \frac{n \eps_\max^2}{r^4}}
\lesssim \sqrt{\frac{\I_r}{n}} + \frac{\eps_\max}{\sqrt{n}r^2}
\end{align*}

Now, $\eps_\max \le r^2 \sqrt{\I_r}$ by \eqref{eq:eps_max_at_most_r^2_I}, and so, finally, 
$$\sup_{\eps \le \eps_\max} \left|\frac{1}{n} \sum_{i=1}^n s_r(X_i - \eps) - \E[s_r (x- \eps)] \right| \lesssim \sqrt{\frac{\log \frac{1}{\delta} }{n} \I_r}$$

We really have that $s_r'(x) \ge -\frac{1}{r^2}$. So, there should be some analagous one-sided argument. In particular, we have
$$s_r(X_i - \eps) \le s_r(X_i) + \frac{\eps}{r^2}$$. So,
\begin{align*}
&\mathcal R_{\mathcal F} \le \frac{1}{n} \sqrt{\E_{X} \left[\sup_{\eps \le \eps_\max} \sum_{i=1}^n s_r(X_i - \eps)^2 \right] } \\
&\le \frac{1}{n} \sqrt{\E_X\left[\sup_{\eps \le \eps_\max} \sum_{i=1}^n (s_r(X_i) + \frac{\eps}{r^2})^2 \right] }\\
&\lesssim \frac{1}{n} \sqrt{\E\left[\sum_{i=1}^n s_r(X_i)^2 \right] + \frac{n \eps_\max^2}{r^4}}
\lesssim \sqrt{\frac{\I_r}{n}} + \frac{\eps_\max}{\sqrt{n}r^2}
\end{align*}
So, we get things to work out on the left of the true mean. On the right, the same argument starting from $\eps_\max$ and going backwards works.


\textbf{My understanding of the net argument} First, for any $|\eps| \le r$ with probability at least $1 - \delta$, $$|\frac{1}{n} \sum_{i=1}^n s_r(x_i + \eps) - \E[s_r(x + \eps)]| \le O\left(\sqrt{\frac{\log \frac{1}{\delta} }{n} \I_r} \right)$$

Now, look at intervals of size $\sqrt{\frac{\log \frac{1}{\delta}}{n \I_r}}$ and divide them up into intervals of size $r^2 \sqrt{ \frac{\log \frac{1}{\delta}}{n} \I_r}$. There are $\frac{1}{r^2 \I_r}$ such intervals. Now, $s'_r(x) \le \frac{1}{r^2}$ for any $x$. So, with probability $1 - \delta \cdot \frac{1}{r^2 \I_r}$, we have that for 


\textbf{Another example, Gaussian with bump} Suppose we have a mixture of standard Gaussian, and Gaussian that is $n^{0.49}$ away and has $1/n$ mass. It will not shift mean or standard deviation by much, but, we will not see it in the KDE stage, but will see a sample in the second stage. The score of this sample will be $~\frac{n^{0.49}}{r^2}$. So it will shift the empirical score by $\frac{n^{-0.51}}{r^2} = n^{-0.01}?$.

%How do we get rid of this $2^k$??
%
%XXX Jasper:
%Choose $x = \frac{1}{2}(\frac{k}{2}-1) = 0.5B$.
%So,
%\begin{align*
%e^{-x}(1+\frac{x}{B})^{B} &= (\frac{1.5}{\sqrt{e}})^B\\
%&\le (0.91)^B \le 0.91
%\end{align*}
%when $k \ge 3$.
%
%For ease of exposition, let $2/k = a \le 1$. Note that: for $x = B^{1-a} / a$, as long as $B^a a \geq 1$,
%\[
%(B + x)^a = B^a \cdot (1 + 1/(B^a a))^a \geq B^a  e^{\frac{1}{2 B^a}} \geq B^a + 1/2.
%\]
%Therefore $e^{-t^a}$ changes by a factor $1/e$ from $t = B$ to $t = B+x$.  So,
%
%\begin{align*}
%\int_{B}^\infty e^{-t^{2/k} r^2} dt &= \int_B^\infty e^{-t^a r^2} dt\\
%&= \sum_{i=0}^\infty \int_{B+ix}^{B+(i+1)x} e^{-t^a r^2 } dt\\
%&\le \sum_{i=0}^\infty x e^{-(B + i x)^a r^2} \\
%&\le x e^{-B^a r^2} \sum_{i=0}^\infty e^{-\frac{i}{2} r^2}\\
%&= x e^{-B^a r^2} \frac{1}{1 - e^{-r^2/2}}\\
%&\lesssim \frac{2 x}{r^2} e^{-B^a r^2}
%\end{align*}
%
%So, $$\E[|u(x)|^k \1_{x \in S}] \lesssim \beta B + \frac{B}{a B^a r^2} e^{-B^a r^2}$$
%Now, let $B^a = \gamma$ be the solution to $$\beta B = \frac{B}{a B^a r^2} e^{-B^a r^2}$$
%This is the same as
%$$B^a r^2 + \log (B^a r^2) = \log \frac{1}{a \beta}$$
%
%So, we have that $$\gamma \le \frac{1}{r^2} \log \frac{1}{a \beta}$$
%
%Now, we will set $B^a = \max\left\{\gamma, \frac{k}{r^2} \right\}$. So, $B^a a \ge \frac{k}{r^2} \cdot \frac{2}{k} \ge 1$ for $r \le 1$. Then, 
%Let $2/k = a$. $B/(a B^a) $ is the size of region needed to shrink by factor $e$. So, 
%
%Setting $B = \frac{\log^{k/2} \frac{k^{k/2}}{\beta}}{r^k }$ gives 
%$$\E[|u(x)|^k \1_{x \in S}] \lesssim \frac{\beta k^k}{r^k} \log^{k/2} \frac{1}{\beta}$$.
%
%Alternatively:
%
%Define $a = 2/k \leq 1$.  Note that: for $x = B^{1-a} / a$, as long as $B^a a \geq 1$,
%\[
%(B + x)^a = B^a \cdot (1 + 1/(B^a a))^a \geq B^a  e^{\frac{1}{2 B^a}} \geq B^a + 1/2.
%\]
%Therefore $e^{-t^a}$ changes by a factor $1/e$ from $t = B$ to $t = B+x$.  So we should expect that
%\[
%\int_B^\infty e^{-t^a} dt \lesssim x e^{-B^a}.
%\]
%[Formally, you could do something like: 
%\[
%\sum_{i=0}^\infty \int_{B+i x}^{B + (i+1)x} \text{blah}.
%\]
%]
%Then we have a bound of:
%\[
%\beta B + \frac{c B^{1 - a}}{a} e^{-B^a}.
%\]
%The first term is increasing in $B$ and the second is decreasing, so we want them to be the same, or
%\[
%\beta = \frac{e^{-B^a}}{a B^a}
%\]
%or essentially
%\[
%B^a = c\log \frac{1}{a \beta},
%\]
%which gives an overall bound of
%\[
%\beta c^{1/a} \log^{1/a} \frac{1}{a \beta} + \beta^c a^{c-1} \log^{1/a - 1} \frac{1}{a \beta}.
%\]
%[NOTE: this required $B^a a \geq 1$, which is often not true.]
%
%Setting $c = 2$ and $a = 2/k$, this is
%\[
%2^{k/2}
%\]
%
%Set $B^a a = 1$ when 
%
%Set $B = \max((c\log \frac{1}{a \beta})^{1/a}, k^{k/2})$.
%Point being that we always set $B$ such that $aB^a \ge 1$, so that the linearisation holds.
%Then ``bound" can be upper bounded by
%$\beta \max(c^{1/a} \log^{1/a} \frac{1}{a \beta},k^{k/2}) + \max(\beta^c a^{c-1} \log^{1/a - 1} \frac{1}{a \beta}, ??)$
%
%XXX Shivam:
%This holds when $$a B^a \ge 1$$ so that $$\beta \lesssim \frac{2}{k} e^{-\frac{k}{2c}}$$
%
%XXX new scratch from Jasper:
%$e^{-t^{2/k}}$ at $t = k^{k/2}$ is equal to $e^{-k}$
%If $B = k^{k/2}$ and $a = 2/k$ then $B^a = k \ge k/2$.
%
%XXX Shivam:
%Let $B^a = \gamma$ be the solution to $$\beta B = \frac{B^{1-a}}{a} e^{-B^a}$$
%This is the same as $$B^a + \log B^a = \log \frac{1}{a\beta}$$
%So, we have that $$\gamma \le \log \frac{1}{a \beta}$$
%Now, we will let $B^a = \max\left{\gamma , k  \right\}$. Then, $B^a a \ge 1$, and we have
%
\begin{lemma}[$kth$ power generic error estimate over large density region]

\end{lemma}
\begin{proof}
\end{proof}

\subsection{Rademacher complexity with Catoni}
First use the KDE analysis to get a good enough estimate so that the $4$th moment of $\Tilde u$ is close to the truth. Use Jasper/Paul's estimator to estimate $\I_r$ from $N = o(n)$ samples using this $\Tilde u$ (that is, use the estimator on $\Tilde u(X_1)^2, \dots, \Tilde u(X_N)^2$). Since the $4th$ moment is $O(\I_r^2)$, we have that this estimator will give us an estimate with error $$O\left(\I_r \sqrt{\frac{\log \frac{1}{\delta}}{N}}\right)$$
with probability $1 - \delta$. Now, if $\frac{\log \frac{1}{\delta}}{N} \to 0$, this is $o(\I_r)$. So, we can estimate the variance of the score (which is equal to $\I_r$) to within $o(\I_r)$.

Using this estimate (call it $v$), we will show that given $n$ samples, for every $\eps \le \eps_\max$ simultaneously, the Catoni estimator gives an estimate of $\E_{x \sim f^*} [u(x - \eps)]$ to within $$\sqrt{\frac{\log \frac{1}{\delta}}{n} \I_r}$$
with probability $1 - \delta$.

Let $\psi(x)$ be the Catoni $\psi$-function. That is $\psi(x)$ is a non-decreasing function with
$$-\log (1 - y +y^2/2)\le \psi(y) \le \log(1 + y + y^2/2)$$

Let $$\phi_\theta(y) =\frac{1}{\alpha} \psi(\alpha(y - \theta)) $$
We will show that with probability $1-\delta$,
$$\sup_{\eps \le \eps_\max} |\frac{1}{n} \sum_{i=1}^n \phi_\theta(\Tilde u(Y_i - \eps)) - (\E_{x \sim f^*}[\Tilde u(x - \eps)] - \theta)| \le \frac{\alpha}{2} \left[v + \left( \frac{\eps_\max}{r^2} - \theta\right)^2 \right] + \frac{\log \frac{1}{\delta}}{n \alpha} + o\left(\sqrt{\frac{\I_r\log\frac{1}{\delta}}{n}} \right)$$

First, we have that pointwise, for any $\eps \le \eps_\max$, using the Chernoff bound, with probability $1-\delta$,
$$|\frac{1}{n} \sum_{i=1}^n \phi_\theta(\Tilde u(Y_i - \eps)) - (\E_{x \sim f^*}[\Tilde u(x - \eps)] - \theta)| \le \frac{\alpha}{2} \left[v + \left( \frac{\eps_\max}{r^2} - \theta\right)^2 \right] + \frac{\log \frac{1}{\delta}}{n \alpha}$$
So, by the Rademacher argument,
$$\sup_{\eps \le \eps_\max} |\frac{1}{n} \sum_{i=1}^n \phi_\theta(\Tilde u(Y_i - \eps)) - (\E_{x \sim f^*}[\Tilde u(x - \eps)] - \theta)| \le \frac{\alpha}{2} \left[v + \left( \frac{\eps_\max}{r^2} - \theta\right)^2 \right] + \frac{\log \frac{1}{\delta}}{n \alpha} + 2 \mathcal R_{\mathcal F}$$
where
$$\mathcal{R}_{\mathcal F} = \E_{Y, \sigma}\left[\sup_{\eps \le \eps_\max} \frac{1}{n} \sum_{i=1}^n \sigma_i \phi_\theta(\Tilde u(Y_i - \eps)) \right]$$
Note that $\phi_\theta$ is $1$-Lipschitz. This is because $\psi(x)$ is $1$-Lipschitz, so that $\psi(\alpha(x - \theta))$ is $\alpha$-Lipschitz, so that $\frac{1}{\alpha} \psi(\alpha(x - \theta))$ is $1$-Lipschitz. So, by Talagrand's contraction lemma,
$$\mathcal R_{\mathcal F} \le \E_{Y, \sigma} \left[\sup_{\eps \le \eps_\max} \frac{1}{n} \sum_{i=1}^n \sigma_i \Tilde u(Y_i - \eps)  \right]$$

\subsection{Net argument using Catoni}
\begin{lemma}[From (XXX Previous paper)]
For any $r$-smoothed distribution $f_r$, $s_r'(x) \ge -\frac{1}{r^2}$, where $s_r$ is the score function of $f_r$.
\end{lemma}
\begin{corollary}
    Our clipped KDE score estimate $\Tilde{u}$ has, for all $x$,
    $$\Tilde u(x - \eps) \le \Tilde u(x) + \frac{\eps}{r^2}$$
\end{corollary}
\begin{proof}
$\Tilde u$ is a clipped version of $\hat u$, the score function of an $r$-smoothed distribution.
\end{proof}

Let $\psi$ be a $1$-Lipschitz Catoni influence function. Let $$\phi_\theta(y) = \frac{1}{\alpha} \psi(\alpha(y - \theta))$$

Since $\psi$ is $1$-Lipschitz, $\phi_\theta(y)$ is $1$-Lipschitz. So, we have that $$\phi_\theta(\Tilde u(x - \eps)) \le \phi_\theta(\Tilde u(x)) + \frac{\eps}{r^2}$$

Let the score estimate at $x$ from apply the Catoni estimator be $\hat \theta(x)$. (This is the estimate from taking $n$ samples $Y_1, \dots, Y_n$, and solving the influence equation at $x$). 
\begin{lemma}[Catoni estimate of score is one-sided Lipschitz]
$$\hat \theta(x-\eps) \le \hat \theta(x) + \frac{\eps}{r^2}$$
\end{lemma}

\begin{proof}
 
\end{proof}




==> original_score_lipschitzness.tex <==
\section{Lipschitzness of the original score}

The goal of this section is to show Lemma~\ref{lem:IntervalBoundSingleScoreFirstDerivative}, which states that, with high probability over sampling $x \from f_r$, it will be the case that $u'(x+\eps)$ is bounded simultaneously for all $\eps \in [\pm r]$.

%\begin{fact}[Scores are bounded with high probability, follows from Section 19]
%Suppose $f$ is an $r$-smoothed distribution, with likelihood $l(\theta,X) = f(X-\theta)$.
%Given a width parameter $\eps_{\max}$, we assume that $r > ??$.
%There exists a constant $\zeta$ such that, for all $\delta \in (0,0.5)$ and for all $\theta \in [\lambda-\eps_{\max}, \lambda+\eps_{\max}]$, with probability at least $1-\delta$ over $n$ samples $x_1,\ldots,x_n \from D_{\lambda}$, we have for every $i \in [n]$ that $\left|\frac{\partial}{\partial \theta} l(\theta,x_i)\right|_{\theta} \le \frac{\zeta}{r}\sqrt{\log\frac{n}{\delta}}$
%\end{fact}

The strategy we use is to in fact prove only pointwise high probability bounds on these derivatives, but instead prove it for a smoothing radius of $1.1r$ as opposed to $r$, and then relate these pointwise bounds to the bounds of over a small interval (of width $r$) with smoothing radius $r$ itself.

The first part consists of the following lemmas on the derivatives/moments.

\begin{proposition}
\label{prop:FirstMomentMixtureHighProbBound}
Let $f$ be an arbitrary distribution and let $f_r$ be the $r$-smoothed version of $f$.
That is, $f_r(x) = \E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}]$.
With probability at least $1-2\delta$ over sampling a point $x \from f_r$, we have
\[ \frac{\E_{y \from f}\left[\max(\frac{|x-y|}{r^2},\frac{1}{r})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)} \le \frac{2\sqrt{6}}{r}\sqrt{\log\frac{1}{\delta}} \] 
\end{proposition}

\begin{proposition}
\label{prop:SecondMomentMixtureHighProbBound}
Let $f$ be an arbitrary distribution and let $f_r$ be the $r$-smoothed version of $f$.
That is, $f_r(x) = \E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}]$.
With probability at least $1-2\delta$ over sampling a point $x \from f_r$, we have
\[ \frac{\E_{y \from f}\left[\max(\frac{|x-y|^2}{r^4},\frac{1}{r^2})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)} \le \frac{14}{r^2}\log\frac{1}{\delta} \] 
\end{proposition}

The proofs of the above propositions are nearly identical, relying on the following lemmas.

%\begin{lemma}
%Consider the distribution $f_r$ which is the $r$-smoothed version of distribution $f$.
%That is, $f_r$ has density $f_r(x) = \E_{y \from h}[\frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}]$.
%Then, with probability at least $1-(1+\tau)\delta$, 	we sample a point $x \from f_r$ such that \[\E_{y \from h}\left[\1\left[(x-y)^2 > 4r^2\log\frac{1}{\delta}\right] \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right] \le \frac{1}{\tau} \E_{y \from h}\left[\1\left[(x-y)^2 \le 4r^2\log\frac{1}{\delta}\right] \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\]
%That is, at least $\frac{\tau}{\tau+1}$ fraction of the density at $x$ comes from Gaussians that are within $2r\sqrt{\log\frac{1}{\delta}}$ of $x$.
%\end{lemma}
%
%\begin{proof}
%	Observe that, at any point $x$ violating the above inequality, we have
%	\begin{align*}
%		f(x) &= \E_{y \from h}\left[\1\left[(x-y)^2 \le 4r^2\log\frac{1}{\delta}\right] \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
%		&\;\;+ \E_{y \from h}\left[\1\left[(x-y)^2 > 4r^2\log\frac{1}{\delta}\right] \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
%		&\le (1+\tau)\E_{y \from h}\left[\1\left[(x-y)^2 > 4r^2\log\frac{1}{\delta}\right] \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]
%	\end{align*}
%	Further observe that
%	\begin{align*}
%		&\int \E_{y \from h}\left[\1\left[(x-y)^2 > 4r^2\log\frac{1}{\delta}\right] \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right] \, \d x\\
%		=& \E_{y \from h}\left[\int \1\left[(x-y)^2 > 4r^2\log\frac{1}{\delta}\right] \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\, \d x\right]\\
%		\le& \E_{y\from h}[\delta] = \delta
%	\end{align*}
%	
%	Thus the probability of sampling a point $x$ violating the lemma inequality is upper bounded by the integral of $f(x)$ over those points, which is in turn upper bounded by $(1+\tau)\delta$.
%\end{proof}

\begin{lemma}
\label{lem:FirstMomentMixturePortion}
Consider the distribution $f_r$ which is the $r$-smoothed version of distribution $f$.
That is, $f_r$ has density $f_r(x) = \E_{y \from h}[\frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}]$.
Then, with probability at least $1-(1+\tau)\delta$, 	we sample a point $x \from f_r$ such that
\begin{align*}  	
&\E_{y \from f}\left[\1\left[(x-y)^2 > 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
\le\;&\frac{1}{\tau} \E_{y \from f}\left[\1\left[(x-y)^2 \le 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]
\end{align*}
\end{lemma}

\begin{proof}
	Observe that, at any point $x$ violating the above inequality, we have
	\begin{align*}
		f_r(x) &= \E_{y \from f}\left[\1\left[(x-y)^2 \le 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right)\frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
		&\;\;+ \E_{y \from f}\left[\1\left[(x-y)^2 > 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right)\frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
		&\le (1+\tau)\E_{y \from f}\left[\1\left[(x-y)^2 > 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]
	\end{align*}
	Further observe that
	\begin{align*}
		&\int \E_{y \from f}\left[\1\left[(x-y)^2 > 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right] \, \d x\\
		=& \E_{y \from f}\left[\int \1\left[(x-y)^2 > 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\, \d x\right]\\
		\le& \E_{y\from f}[\delta] = \delta
	\end{align*}
	
	Thus the probability of sampling a point $x$ violating the lemma inequality is upper bounded by the integral of $f_r(x)$ over those points, which is in turn upper bounded by $(1+\tau)\delta$.
\end{proof}

\begin{lemma}
\label{lem:SecondMomentMixturePortion}
Consider the distribution $f_r$ which is the $r$-smoothed version of distribution $f$.
That is, $f_r$ has density $f_r(x) = \E_{y \from h}[\frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}]$.
Then, with probability at least $1-(1+\tau)\delta$, 	we sample a point $x \from f_r$ such that
\begin{align*}  	
&\E_{y \from f}\left[\1\left[(x-y)^2 > 7r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|^2}{r^4},\frac{1}{r^2}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
\le\;&\frac{1}{\tau} \E_{y \from f}\left[\1\left[(x-y)^2 \le 7r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|^2}{r^4},\frac{1}{r^2}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]
\end{align*}
\end{lemma}

\begin{proof}
	Observe that, at any point $x$ violating the above inequality, we have
	\begin{align*}
		f_r(x) &= \E_{y \from f}\left[\1\left[(x-y)^2 \le 7r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|^2}{r^4},\frac{1}{r^2}\right)\frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
		&\;\;+ \E_{y \from f}\left[\1\left[(x-y)^2 > 7r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|^2}{r^4},\frac{1}{r^2}\right)\frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
		&\le (1+\tau)\E_{y \from f}\left[\1\left[(x-y)^2 > 7r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|^2}{r^4},\frac{1}{r^2}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]
	\end{align*}
	Further observe that
	\begin{align*}
		&\int \E_{y \from f}\left[\1\left[(x-y)^2 > 7r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|^2}{r^4},\frac{1}{r^2}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right] \, \d x\\
		=& \E_{y \from f}\left[\int \1\left[(x-y)^2 > 7r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|^2}{r^4},\frac{1}{r^2}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\, \d x\right]\\
		\le& \E_{y\from f}[\delta] = \delta
	\end{align*}
	
	Thus the probability of sampling a point $x$ violating the lemma inequality is upper bounded by the integral of $f_r(x)$ over those points, which is in turn upper bounded by $(1+\tau)\delta$.
\end{proof}

With the above 2 lemmas, we can prove Propositions~\ref{prop:FirstMomentMixtureHighProbBound} and~\ref{prop:SecondMomentMixtureHighProbBound}.

\begin{proof}[Proof of Propositions~\ref{prop:FirstMomentMixtureHighProbBound}, and \ref{prop:SecondMomentMixtureHighProbBound}]
	The proofs of the two propositions are identical and we prove only Proposition~\ref{prop:FirstMomentMixtureHighProbBound}.
	
	By Lemma~\ref{lem:FirstMomentMixturePortion}, with probability $1-2\delta$ over sampling a single point $x \from f_r$, the point $x$ satisfies 
	\begin{align*}  	
&\E_{y \from f}\left[\1\left[(x-y)^2 > 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]\\
\le\;& \E_{y \from f}\left[\1\left[(x-y)^2 \le 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]
	\end{align*}
	
	And so,
	\begin{align*}
	&\frac{\E_{y \from f}\left[\max(\frac{|x-y|}{r^2},\frac{1}{r})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\\
	=\;& \frac{\E_{y \from f}\left[\1\left[(x-y)^2 \le 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\\
	+& \frac{\E_{y \from f}\left[\1\left[(x-y)^2 > 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\\
	\le\;& 2\cdot \frac{\E_{y \from f}\left[\1\left[(x-y)^2 \le 6r^2\log\frac{1}{\delta}\right] \max\left(\frac{|x-y|}{r^2},\frac{1}{r}\right) \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\\
	\le\;& \frac{2\sqrt{6}}{r}\sqrt{\log\frac{1}{\delta}}\frac{\E_{y \from f}\left[\1\left[(x-y)^2 \le 6r^2\log\frac{1}{\delta}\right] \frac{1}{\sqrt{2\pi r^2}} e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\\
	\le\;& \frac{2\sqrt{6}}{r}\sqrt{\log\frac{1}{\delta}}
	\end{align*}

\end{proof}

The next step is to generalise Propositions~\ref{prop:FirstMomentMixtureHighProbBound} and~\ref{prop:SecondMomentMixtureHighProbBound} to a high probability guarantee over the interval $[x-r,x+r]$ from sampling $x \from f_r$.
The technique is to relate the interval versions of the propositions with respect to $r$-smoothing to the propositions with respect to $\sqrt{1.1}r$-smoothing.

We will use the following basic fact.

\begin{fact}
\label{fact:MixtureRatio}
	Consider a non-decreasing sequence of fractions $\frac{a_1}{b_1} \le \ldots \frac{a_k}{b_k}$ where all $a_i$ and $b_i$ are non-negative, and an arbitrary non-negative sequence $\{\gamma_i\}$.
	Suppose there is another non-negative sequence $\{c_i\}$ that is also non-decreasing.
	Then,
	\[ \frac{\sum_i \gamma_i a_i}{\sum_i \gamma_i b_i} \le \frac{\sum_i \gamma_i c_i a_i}{\sum_i \gamma_i c_i b_i} \]
	This fact can be generalized to arbitrary mixture measures instead of finite discrete measures.
\end{fact}

We will also use the following notation:

\[ c_r(x,\eps) = \frac{e^{-\frac{x^2}{2.2r^2}}}{e^{-\frac{(x+\eps)^2}{2r^2}}} = e^{\frac{\eps^2}{2r^2}} e^{\frac{1}{22r^2}x(x+22\eps)}\]

Using the above fact and notation, we show deterministic inequalities relating the quantities bounded in Propositions~\ref{prop:FirstMomentMixtureHighProbBound} and~\ref{prop:SecondMomentMixtureHighProbBound} \emph{over an entire interval} to the same quantities over a single point, but using $f_{\sqrt{1.1}r}$ instead of $f_r$.

\begin{proposition}
\label{prop:WidenFirstMomentMixture}
Let $f$ be an arbitrary distribution and let $f_r$ be the $r$-smoothed version of $f$.
That is, $f_r(x) = \E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}]$.
For any point $x \in \R$ and any $|\eps| \le r$, we have
\[ \frac{\E_{y \from f}\left[\max(\frac{|x+\eps-y|}{r^2},\frac{1}{r})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{f_r(x+\eps)} \le 132 \cdot  \frac{\E_{y \from f}\left[\max(\frac{|x-y|}{1.1r^2},\frac{1}{r\sqrt{1.1}})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{f_{\sqrt{1.1}r}(x)}\] 
\end{proposition}

\begin{proof}
	First, observe that the expression $\max(\frac{|z+\eps|}{r^2},\frac{1}{r})$ is always upper bounded by $22\max(\frac{\sqrt{z(z+22\eps)}}{r^2},\frac{1}{r})$ for $|\eps| \le r$ (which can be checked on MATLAB, by factoring out the $\frac{1}{r}$ and reparametrising $z$ and $\eps$ in the $r$-scale).
	Thus,
	\begin{align*}
	&\frac{\E_{y \from f}\left[\max(\frac{|x+\eps-y|}{r^2},\frac{1}{r})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{f_r(x+\eps)}\\
	\le\;& 22\cdot\frac{\E_{y \from f}\left[\max(\frac{\sqrt{(x-y)(x-y+22\eps)}}{r^2},\frac{1}{r})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{\E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}]}
	\end{align*}
	
	Next, we use Fact~\ref{fact:MixtureRatio} using the fractions $a_i/b_i$ equalling $\max(\frac{\sqrt{(x-y)(x-y+22\eps)}}{r^2},\frac{1}{r})$, and the $c_i$ equalling $c_r(x-y,\eps)$, using the fact that both expressions are increasing in $(x-y)(x-y+22\eps)$, which upper bounds the above quantity by
	\begin{align*}
	&22\cdot\frac{\E_{y \from f}\left[\max(\frac{\sqrt{(x-y)(x-y+22\eps)}}{r^2},\frac{1}{r})\frac{c_r(x-y,\eps)}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{\E_{y \from f}[\frac{c_r(x-y,\eps)}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}]}\\
	=\;& 22\cdot\frac{\E_{y \from f}\left[\max(\frac{\sqrt{(x-y)(x-y+22\eps)}}{r^2},\frac{1}{r})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{\E_{y \from f}[\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}]}
	\end{align*}
	
	Lastly, we observe that $\max(\frac{\sqrt{z(z+22\eps)}}{r^2},\frac{1}{r}) \le 6\max(\frac{|z|}{1.1r^2},\frac{1}{r\sqrt{1.1}})$, which allows us to prove the proposition by bounding the last quantity by
	\[ 132 \cdot \frac{\E_{y \from f}\left[\max(\frac{|x-y|}{1.1r^2},\frac{1}{r\sqrt{1.1}})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{f_{\sqrt{1.1}r}(x)} \]
\end{proof}

\begin{proposition}
\label{prop:WidenSecondMomentMixture}
Let $f$ be an arbitrary distribution and let $f_r$ be the $r$-smoothed version of $f$.
That is, $f_r(x) = \E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}]$.
For any point $x \in \R$ and any $|\eps| \le r$, we have
\[ \frac{\E_{y \from f}\left[\max(\frac{|x+\eps-y|^2}{r^4},\frac{1}{r^2})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{f_r(x+\eps)} \le 12000 \cdot  \frac{\E_{y \from f}\left[\max(\frac{|x-y|^2}{1.1^2r^4},\frac{1}{r^2})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{f_{\sqrt{1.1}r}(x)}\] 
\end{proposition}

\begin{proof}
	First, observe that the expression $\max(\frac{|z+\eps|^2}{r^4},\frac{1}{r^2})$ is always upper bounded by $444\max(\frac{z(z+22\eps)}{r^4},\frac{1}{r^2})$ for $|\eps| \le r$.
	Thus,
	\begin{align*}
	&\frac{\E_{y \from f}\left[\max(\frac{|x+\eps-y|^2}{r^4},\frac{1}{r^2})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{f_r(x+\eps)}\\
	\le\;& 444\cdot\frac{\E_{y \from f}\left[\max(\frac{(x-y)(x-y+22\eps)}{r^4},\frac{1}{r^2})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{\E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}]}
	\end{align*}
	
	Next, we use Fact~\ref{fact:MixtureRatio} using the fractions $a_i/b_i$ equalling $\max(\frac{(x-y)(x-y+22\eps)}{r^4},\frac{1}{r^2})$, and the $c_i$ equalling $c_r(x-y,\eps)$, using the fact that both expressions are increasing in $(x-y)(x-y+22\eps)$, which upper bounds the above quantity by
	\begin{align*}
	&444\cdot\frac{\E_{y \from f}\left[\max(\frac{(x-y)(x-y+22\eps)}{r^4},\frac{1}{r^2})\frac{c_r(x-y,\eps)}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{\E_{y \from f}[\frac{c_r(x-y,\eps)}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}]}\\
	=\;& 444\cdot\frac{\E_{y \from f}\left[\max(\frac{(x-y)(x-y+22\eps)}{r^4},\frac{1}{r^2})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{\E_{y \from f}[\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}]}
	\end{align*}
	
	Lastly, we observe that $\max(\frac{z(z+22\eps)}{r^4},\frac{1}{r^2}) \le 27\max(\frac{|z|^2}{1.1^2r^4},\frac{1}{1.1r^2})$, which allows us to prove the proposition by bounding the last quantity by
	\[ 12000 \cdot \frac{\E_{y \from f}\left[\max(\frac{|x-y|^2}{1.1^2r^4},\frac{1}{1.1r^2})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{f_{\sqrt{1.1}r}(x)} \]
\end{proof}



Lastly, we relate the probability of events under $f_r$ and $f_{\sqrt{1.1}r}$ and show that they are quadratically related.

\begin{proposition}
	Let $G_r$ be the Gaussian measure with standard deviation $r$.
	Then, for any measurable set $S \subseteq \R$, we have
	\[ G_r(S) \le \sqrt{2G_{\sqrt{1.1}r}(S)} \]
\end{proposition}

\begin{proof}
Given the scale-invariance of the claim, we show this for $r=1$ for notational simplicity, and denote $G = G_1$.
First, we note that the chi-square divergence $\chi^2(G \, || \, G_{\sqrt{1.1}})$ is a constant much less than 1 (in particular, less than 0.5).

The variational representation of $\chi^2(P \, || \, Q)$ is $\sup_{h : \mathcal{X} \to \R} 2\E_{x \from P}[h(x)] - \E_{x \from Q}[h^2(x)] - 1$.
Choosing $h(x) = \1[x \in S]/G(S)$ for $P = G$, $Q = G_{\sqrt{1.1}}$, the expression inside the supremum evaluates to
\[ 2\frac{G(S)}{G(S)} - \frac{G_{\sqrt{1.1}}(S)}{G^2(S)} - 1 \]
which is equal to $1 - \frac{G_{\sqrt{1.1}}(S)}{G^2(S)}$, which by the supremum definition is upper bounded by $\chi^2(G \, || \, G_{\sqrt{1.1}}) < 0.5$.

Therefore, $\frac{G_{\sqrt{1.1}}(S)}{G^2(S)} \ge \frac{1}{2}$, implying that $G(S) \le \sqrt{2G_{\sqrt{1.1}}(S)}$.	
\end{proof}

\begin{corollary}
\label{cor:WidenSmoothingProb}
	Consider $f_r$, the $r$-smoothed version of distribution $f$.
	Then, for any measurable set $S \subseteq \R$, we have
	\[ f_r(S) \le \sqrt{2f_{\sqrt{1.1}r}(S)} \]
\end{corollary}

\begin{proof}
Generalizing the previous proposition to a Gaussian mixtures $f_r$ and $f_{\sqrt{1.1}r}$, we know that $f_r(S) = \E_{y \from f}[G_r(S-y)] \le \E_{y \from f}[\sqrt{2G_{\sqrt{1.1}}(S-y)}] \le \sqrt{2\E_{y \from f}[G_{\sqrt{1.1}r}(S-y)]} = \sqrt{2f_{\sqrt{1.1}r}(S)}$
where the second inequality is an application of Jensen's inequality using the concavity of the square root.
\end{proof}

We are now ready to state and prove the interval versions of Propositions~\ref{prop:FirstMomentMixtureHighProbBound} and~\ref{prop:SecondMomentMixtureHighProbBound}.

\begin{proposition}
\label{prop:IntervalFirstMomentMixtureHighProbBound}
Let $f$ be an arbitrary distribution and let $f_r$ be the $r$-smoothed version of $f$.
That is, $f_r(x) = \E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}]$.
With probability at least $1-\delta$ over sampling a point $x \from f_r$, we have that for all $|\eps| \le r$,
\[ \frac{\E_{y \from f}\left[\max(\frac{|x+\eps-y|}{r^2},\frac{1}{r})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{f_r(x+\eps)} \le \frac{840}{r}\sqrt{\log\frac{2}{\delta}} \] 
\end{proposition}

\begin{proof}
By Proposition~\ref{prop:FirstMomentMixtureHighProbBound}, with probability at least $1-\frac{\delta^2}{2}$ over the sampling of $x \from f_{\sqrt{1.1}r}$, the point $x$ satisfies

\[ \frac{\E_{y \from f}\left[\max(\frac{|x-y|}{1.1r^2},\frac{1}{r\sqrt{1.1}})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{f_{\sqrt{1.1}r}(x)} \le \frac{4\sqrt{3}}{r\sqrt{1.1}}\sqrt{\log\frac{2}{\delta}} \] 

By Corollary~\ref{cor:WidenSmoothingProb}, the same holds for sampling $x \from f_r$ with probability at least $1-\delta$.

Finally, by Proposition~\ref{prop:WidenFirstMomentMixture}, we know that if the above event happens for point $x$, then it implies that for all $|\eps| \le r$, we have 
\begin{align*}
&\frac{\E_{y \from f}\left[\max(\frac{|x+\eps-y|}{r^2},\frac{1}{r})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{f_r(x+\eps)}	\\
\le\;& 132\cdot \frac{\E_{y \from f}\left[\max(\frac{|x-y|}{1.1r^2},\frac{1}{r\sqrt{1.1}})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{f_{\sqrt{1.1}r}(x)}\\
<\;& \frac{840}{r}\sqrt{\log\frac{2}{\delta}}
\end{align*}
thus proving the proposition.
\end{proof}

\begin{proposition}
\label{prop:IntervalSecondMomentMixtureHighProbBound}
Let $f$ be an arbitrary distribution and let $f_r$ be the $r$-smoothed version of $f$.
That is, $f_r(x) = \E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}]$.
With probability at least $1-\delta$ over sampling a point $x \from f_r$, we have that for all $|\eps| \le r$,
\[ \frac{\E_{y \from f}\left[\max(\frac{|x+\eps-y|^2}{r^4},\frac{1}{r^2})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{f_r(x+\eps)} \le \frac{310000}{r^2}\log\frac{2}{\delta} \] 
\end{proposition}

\begin{proof}
By Proposition~\ref{prop:SecondMomentMixtureHighProbBound}, with probability at least $1-\frac{\delta^2}{2}$ over the sampling of $x \from f_{\sqrt{1.1}r}$, the point $x$ satisfies

\[ \frac{\E_{y \from f}\left[\max(\frac{|x-y|^2}{1.1^2r^4},\frac{1}{1.1r^2})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{f_{\sqrt{1.1}r}(x)} \le \frac{28}{1.1r^2}\log\frac{2}{\delta} \] 

By Corollary~\ref{cor:WidenSmoothingProb}, the same holds for sampling $x \from f_r$ with probability at least $1-\delta$.

Finally, by Proposition~\ref{prop:WidenSecondMomentMixture}, we know that if the above event happens for point $x$, then it implies that for all $|\eps| \le r$, we have 
\begin{align*}
&\frac{\E_{y \from f}\left[\max(\frac{|x+\eps-y|^2}{r^4},\frac{1}{r^2})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x+\eps-y)^2}{2r^2}}\right]}{f_r(x+\eps)}	\\
\le\;& 12000\cdot \frac{\E_{y \from f}\left[\max(\frac{|x-y|^2}{1.1r^4},\frac{1}{1.1r^2})\frac{1}{\sqrt{2.2\pi r^2}}e^{-\frac{(x-y)^2}{2.2r^2}}\right]}{f_{\sqrt{1.1}r}(x)}\\
<\;& \frac{310000}{r^2}\log\frac{2}{\delta}
\end{align*}
thus proving the proposition.
\end{proof}

Finally, we can show a high probability bound on the second derivative of the score over an entire interval around a sampled point.

\begin{lemma}
\label{lem:IntervalBoundSingleScoreFirstDerivative}
Let $f$ be an arbitrary distribution and let $f_r$ be the $r$-smoothed version of $f$.
That is, $f_r(x) = \E_{y \from f}[\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}]$.
Let $u_r(x)$ be the score of $f_r$ at point $x$, namely $\frac{d}{dx} \log f_r(x) = \frac{f'_r(x)}{f_r(x)}$.
With probability at least $1-\delta$ over sampling a point $x \from f_r$, we have that for all $|\eps| \le r$,
\[ \left|u'_r(x+\eps)\right| \le \frac{1325600}{r^2}\log\frac{4}{\delta} \]
\end{lemma}

\begin{proof}
First, note that
\[ u'_r(x) = \frac{f''_r(x)}{f_r(x)} - \left(\frac{f'_r(x)}{f_r(x)}\right)^2\]

We will bound the two terms $\frac{f'_r(x)}{f_r(x)}$ and $\frac{f''_r(x)}{f_r(x)}$ individually over the $\pm\eps$ interval around point $x$, and combine using the triangle inequality.

For the first derivative, we have that for all $x$,
\[ \left|\frac{f'_r(x)}{f_r(x)}\right| = \left|\frac{\E_{y \from f}\left[\frac{-(x-y)}{r^2}\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\right| \le \frac{\E_{y \from f}\left[\max(\frac{|x-y|}{r^2},\frac{1}{r})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\]
Thus, by Proposition~\ref{prop:IntervalFirstMomentMixtureHighProbBound}, we know that with probability at least $1-\frac{\delta}{2}$ over sampling $x \from f_r$, we have that for all $|\eps| \le r$,
\[ \left|\frac{f'_r(x+\eps)}{f_r(x+\eps)}\right| \le \frac{840}{r}\sqrt{\log\frac{4}{\delta}} \]

For the second derivative, we have that for all $x$,
\[ \left|\frac{f''_r(x)}{f_r(x)}\right| = \left|\frac{\E_{y \from f}\left[\frac{(x-y)^2-r^2}{r^4}\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\right| \le 2\cdot\frac{\E_{y \from f}\left[\max(\frac{|x-y|^2}{r^4},\frac{1}{r^2})\frac{1}{\sqrt{2\pi r^2}}e^{-\frac{(x-y)^2}{2r^2}}\right]}{f_r(x)}\]
Thus, by Proposition~\ref{prop:IntervalSecondMomentMixtureHighProbBound}, we know that with probability at least $1-\frac{\delta}{2}$ over sampling $x \from f_r$, we have that for all $|\eps| \le r$,
\[ \left|\frac{f''_r(x+\eps)}{f_r(x+\eps)}\right| \le \frac{620000}{r^2}\log\frac{4}{\delta} \]

Concluding, with probability at least $1-\delta$ over sampling $x \from f_r$, all three of the above events hold, meaning that for all $|\eps| \le r$, we have
\begin{align*}
\left|u'_r(x+\eps)\right| &= \left|\frac{f''_r(x+\eps)}{f_r(x+\eps)} - \left(\frac{f'_r(x+\eps)}{f_r(x+\eps)}\right)^2\right|\\
&\le \left|\frac{f''_r(x+\eps)}{f_r(x+\eps)}\right| + \left|\frac{f'_r(x+\eps)}{f_r(x+\eps)}\right|^2\\
&\le \frac{620000 + 840^2}{r^2}\log\frac{5}{\delta}\\
&\le \frac{1325600}{r^2}\log\frac{4}{\delta}
\end{align*}
\end{proof}

==> understanding_moment_problem_kde.tex <==

XXX Notes about understanding moment problem: \textbf{Standard Gaussian case:}
\[
\sqrt{A + B} \approx \sqrt{A} + \sqrt{\frac{B}{2A}}
\]
when $A \gg B$.
\begin{itemize}
    \item If we see $N$ samples, our last sample will be close to $\sqrt{2 \log (N/\sqrt{2\pi})} = \sqrt{2 \log N - O(1)} = \sqrt{2 \log N} - O(1/\sqrt{\log N})$ (since from the uniform distribution on $[0,1]$, the largest sample will be at $\frac{N-1}{N}$ in expectation, so that $F^{-1}(1 - 1/N)$ is the $t$ such that $e^{-t^2} \approx 1/N$).
    
    \item If we care about the $k^{th}$ moment, the expected kth moment is  $\sqrt{k}^k$, so $\E[x^k]$ is mostly coming from $\abs{x} \approx \sqrt{k}$.
    
    \item $\sqrt{\log N}$ = $\sqrt{\log \beta n}$ for constant $\beta < 1$. If the largest sample in the KDE is $\sqrt{\log \beta n}$, we have that the score at $\sqrt{\log n}$ is $\frac{\sqrt{\log n} - \sqrt{\log \beta n}}{r^2} \approx \frac{1}{r^2 \sqrt{\log n}} = n^{\Omega(1)}$ from the KDE, while the true score is $\sqrt{\log n}$.
    
    This is big, but not \emph{that} big.  It's like $n^{1/3}$, and we're averaging over $n$ samples, so to make $\sqrt{\frac{\log (1/\delta)}{n}}$ bias you need $n^{1/6} \sqrt{\log \frac{1}{\delta}}$ such samples.  And I guess there's a $\delta$ chance that you see $\Theta(\log \frac{1}{\delta})$ such large values, which would be a problem if $\log \frac{1}{\delta} > n^{1/3}$, or $n < \log^{3} \frac{1}{\delta}$, which maybe could happen.
    
    In general, seems like a problem if $\sqrt{n \log \frac{1}{\delta}}r^2 < \log \frac{1}{\delta}$, and I think we do want to handle some of this regime?
    
        Or in other words: we can set $r \geq (\frac{\log \frac{1}{\delta}}{n})^{1/4}$ and this particular example does not seem to be a problem.
    
    \item XXX Shivam: rewriting above in different language, we have that with probability $\delta$, we see $\log \frac{1}{\delta}$ samples with score larger than $n^{1/3}$. Now, if this happens, the contribution to the empirical mean is $\frac{n^{1/3} \log \frac{1}{\delta}}{n}$. This is a problem if it is larger than the confidence interval we want, which has width $\sqrt{\frac{\log \frac{1}{\delta}}{n}}$, which means we have a problem when $n < \log^3 \frac{1}{\delta}$. 
    \item Observation: Consider the Pareto distribution with parameter $2 + \gamma$. We have that $$\Pr[X \ge t] \le \frac{1}{t^{2+\gamma}}$$
    Now, we will see $O(N r^{2+\gamma})$ samples between $\frac{1}{r}$ and $\frac{100}{r}$. These samples will have spacing of order $$\frac{1}{r} * \frac{1}{N r^{2+\gamma}} = \frac{1}{N r^{3+\gamma}}$$
    So, there is going to be a large size region with score roughly of order $\frac{1}{N r^{3+\gamma}} * \frac{1}{r^2} = \frac{1}{N r^{5+\gamma}}$.
    In the second stage, we will see $n r^{2+\gamma}$ samples between $\frac{1}{r}$ and $\frac{100}{r}$, and a constant fraction of these will have score $\frac{1}{N r^{5+\gamma}}$. So, the total contribution will be $\frac{n}{Nr^{3+\gamma}}$, and the average contribution will be $\frac{1}{N r^{3+\gamma}}$. When $r > \frac{1}{N^{1/(3+\gamma)}}$, this is small. This says that the problem doesn't seem to be in the tails of the distribution, but rather the center?
    \item Intuition: In the Gaussian case, the bad case was the largest samples being far apart, but clipping fixes this even in the heavy-tailed case. However, in the heavy-tailed case, the distributions are flat, and so the bad case could instead be large contributions from in between the KDE samples.
    
    In the case of the Pareto distribution with parameter $\approx 2$, the samples in the KDE round are going to be placed at roughly $\sqrt{\frac{N}{k}}$ for $k = 1, \dots, N$. So the space between the samples should be $\sqrt{\frac{N}{k - 1}} - \sqrt{\frac{N}{k}} \approx \frac{\sqrt{N}}{k^{3/2}}$. (This is because the samples are sampled from the true distribution $f^*$ and not the KDE, so that we will always see a constant fraction of samples in the center between the two $r$-radius Gaussians. Since $n$ is some large constant times $N$, we can basically assume enough samples hit this region) So, the score contribution of a sample in between these two (in abs value) should be $\frac{\sqrt{N}}{k^{3/2} r^2}$. We will expect to see $n/N$ samples between $\sqrt{\frac{N}{k-1}}$ and $\sqrt{\frac{N}{k}}$. So, the total contribution to score should be $$\frac{n}{\sqrt{N}k^{3/2} r^2}$$
    So, the average contribution is $\frac{1}{\sqrt{N} k^{3/2} r^2}$ from samples between $\sqrt{\frac{N}{k-1}}$ and $\sqrt{\frac{N}{k}}$. We can approximate this by integrating from $1$ to $N$, to get that the average contribution is $\approx \frac{1}{\sqrt{N} r^2}$. So, we have a problem if this is larger than $\sqrt{\frac{\log \frac{1}{\delta}}{n}}$, or when $r \le \frac{1}{\log^{1/4} \frac{1}{\delta}}$, which is basically always the case. OK, but this is not an accurate picture - it's saying that the total contribution of \emph{absolute value} of score in the second stage is $O(\frac{n}{\sqrt{N} r^2})$. However, most of the time, half of this score is positive and half negative. We instead want to say that with good probability, the total score is skewed in one or the other direction so that the estimate is thrown off.
    \item More accurate picture: We have coins, $n/N = C$ coins ($\pm 1$ with $0$ bias) with weight $\frac{\sqrt{N}}{k^{3/2} r^2}$ for every $k = 1\dots N$. We want to know how large the bias can be with probability $1 - \delta$.
    
    Idea: Divide into $\log n$ groups of size powers of $2$, and understand concentration of each group.
    
    \item  Question: suppose you have $n$ coins with probability $p = n^{-2/3}$.  The number of heads has about a $1/n$ chance of being what?
    
    Basically like $Poi(n^{1/3})$, so $\Pr[X > t] = e^{-n^{1/3}}n^{t/3}/t! \approx e^{-n^{1/3} + (t/3) \log n - t \log t}$.  For $t = n^{1/2}$, this is $e^{- (t/6) \log n} \gg \delta$.  (This is $\gg \delta$ because $n \approx \log \frac{1}{\delta}$, so this is $e^{-\sqrt{\log (1/\delta)}}$.)
\end{itemize}

